Design and Implementation of an Analysis Pipeline for Heterogeneous Data

Managing and preparing complex data for deep learning, a prevalent approach in large-scale data science can be challenging. Data transfer for model training also presents difficulties, impacting scientific fields like genomics, climate modeling, and astronomy. A large-scale solution like Google Pathways with a distributed execution environment for deep learning models exists but is proprietary. Integrating existing open-source, scalable runtime tools and data frameworks on high-performance computing (HPC) platforms is crucial to address these challenges. Our objective is to establish a smooth and unified method of combining data engineering and deep learning frameworks with diverse execution capabilities that can be deployed on various high-performance computing platforms, including cloud and supercomputers. We aim to support heterogeneous systems with accelerators, where Cylon and other data engineering and deep learning frameworks can utilize heterogeneous execution. To achieve this, we propose Radical-Cylon, a heterogeneous runtime system with a parallel and distributed data framework to execute Cylon as a task of Radical Pilot. We thoroughly explain Radical-Cylon's design and development and the execution process of Cylon tasks using Radical Pilot. This approach enables the use of heterogeneous MPI-communicators across multiple nodes. Radical-Cylon achieves better performance than Bare-Metal Cylon with minimal and constant overhead. Radical-Cylon achieves (4~15)% faster execution time than batch execution while performing similar join and sort operations with 35 million and 3.5 billion rows with the same resources. The approach aims to excel in both scientific and engineering research HPC systems while demonstrating robust performance on cloud infrastructures. This dual capability fosters collaboration and innovation within the open-source scientific research community.

==> tex/discussion.tex <==
\section{Discussions}
\label{sec:discussions}

Cylon-RP results in \ref{subsec:exp-join},~\ref{subsec:exp-sort} show that Radical-Cylon scales efficiently with very small overheads and outperforms MPI-Cylon in ~\ref{subsec:exp-rp-cylon-mpi-cylon}. In specific, RP-Cylon overheads presented in Table~\ref{tab:a-b-exp_table} show that RP-Cylon takes an average of 3.4 seconds to construct an~\texttt{MPI-Communincator} with 518 ranks which are marginal compared to the total execution time and the size of the experiments.

Cylon performance is measured with a data frame execution runtime. A collection of data frame operators can be arranged in a directed acyclic graph (DAG). Execution of this DAG can further be improved by identifying independent branches of execution and executing such independent tasks parallelly. Additionally, each of these tasks themselves is Bulk Synchronize Parallel (BSP) (this is not the case in most of the engines that are available today). RP-Cylon integration allows us to control the parallelism of these BSP tasks. 
In the future, Cylon is planning to add an optimizer based on the data frame DAG. One aspect is traditional query optimization, similar to SQL query optimization, which is orthogonal to the scheduling mechanism. Another important metric would need would be, what is the scheduling overhead distribution of the underlying scheduling environment.

RP has been meticulously crafted to address a unified execution setting encompassing both CPUs and GPUs, catering to the needs of multiple data pipelines. While integrating CPUs and GPUs within a single task does introduce computational intricacies owing to the foundational structure of Cylon, the concept of heterogeneous execution remains viable. This involves employing distinct groups of ranks equipped with specialized memory allocated either on CPUs or GPUs, enabling the concurrent utilization of these processing units.

The design of RADICAL-Pilot aims to support an extensive spectrum of meticulous resource management policies. Our initial focus has revolved around establishing multiple data pipelines and executing distributed operations in the form of functions. Here Cylon plays an important part by providing distributed execution. Looking ahead to more complex multi-tenancy scenarios, RADICAL-Pilot must proficiently manage a diverse range of resource types, including not only device and host memory but also network bandwidth. The Master-Worker raptor model employed by RADICAL-Pilot provides the system with a robust capability to monitor available resources and allocate them on a large scale. Our future plans involve exploring common multi-tenancy requirements such as prioritization, performance segregation, and resource tracking. Importantly, the timeframe for these endeavors will be considerably shorter than prior efforts yet will encompass significantly larger pools of resources.


